Lambda Learner: Fast Incremental Learning on Data Streams

One of the most well-established applications of machine learning is in deciding what content to show website visitors. When observation data comes from high-velocity, user-generated data streams, machine learning methods perform a balancing act between model complexity, training time, and computational costs. Furthermore, when model freshness is critical, the training of models becomes time-constrained. Parallelized batch offline training, although horizontally scalable, is often not time-considerate or cost-effective. In this paper, we propose Lambda Learner, a new framework for training models by incremental updates in response to mini-batches from data streams. We show that the resulting model of our framework closely estimates a periodically updated model trained on offline data and outperforms it when model updates are time-sensitive. We provide theoretical proof that the incremental learning updates improve the loss-function over a stale batch model. We present a large-scale deployment on the sponsored content platform for a large social network, serving hundreds of millions of users across different channels (e.g., desktop, mobile). We address challenges and complexities from both algorithms and infrastructure perspectives, and illustrate the system details for computation, storage, and streaming production of training data.

==> notes.tex <==


\section{Preso equations}
\begin{alignat}{1}
\label{gen:main-cumxxxulative}
F^{(t)}(\beta) &= \sum_{k=0}^{k=t} \delta^{t-k} f^{(k)}({\beta}) \nonumber\\
& = \delta F^{(t-1)}(\beta) + f^{(t)}(\beta),
\end{alignat}

\begin{alignat}{1}
\label{glmix:mainxx2}
\minimize{\beta} &\,\,\,\,  F^{(t)}(\beta) - \log p(\beta)  \,\,\,\,\,  \left(=\delta F^{(t-1)}(\beta)  + f^{(t)}(\beta) - \log p(\beta)\right),
\end{alignat}
The first term of objective function can be approximated using a quadratic function centered around previous optimum $\beta^{*(t-1)}$,

\begin{alignat}{1}
\label{glmix:maizxxxn3}
\minimize{\beta} &\,\,\,\,   \tfrac{\delta}{2}\|\beta - \beta^{*(t-1)}\|^{2}_{\nabla^{2} F^{(t-1)}(\beta^{*(t-1)})} + f^{(t)}(\beta) + \tfrac{\lambda}{2}\|\beta\|^{2}.
\end{alignat}

% \subsection{Special Case: Hierarchical Random Effect}
% In the case where we have structured random effects for $A$ advertisers, $C$ ad-campaigns, and $c$ ad-creatives, there is a natural hierarchical structure which allows us to split the online traffic, observations data, and model updates for (\ref{glmix:random}) into $A$ independent sub-problems which do not need cross-communication at any time after \textbf{\emph{Step 1}}.

% \subsection{Concept Drift for Existing Items}

% {\color{red} <Open question: what is the difference between covariate shift and concept drift? can we use covariate shift to address concept drift?>}

% Three widely used methods for handling concept drift are: time windows \citep{Widmer:1996}, instance weighting \citep{Klinkenberg:2002}, and ensemble learning \citep{Wang:2003}. In the first method, a time window is applied to the data stream and the data within the window are employed to build the classifier for the current concept. The window keeps moving towards the future so that the most recent recording is always included in the window. The window acts like a limited memory, with the data outside the window forgotten. A key issue is to determine the window size, which should accurately capture the rate of concept drift. The method of instance weighting is based on the observation that the importance of a past example to the current concept does not change abruptly but rather decreases gradually. A weight is assigned to each past example to reflect its importance. Assuming that concept drift is monotonic (i.e., newer examples are always more important than older ones), one can construct the weights according to the age of each example; for example, one can choose weights that decrease exponentially with the age of examples \cite{Klinkenberg:2002}.

% The method of ensemble learning maintains an ensemble of classifiers, instead of a single one, for the current concept. This is done by dividing the data stream into chunks and learning a classifier based on each data chunk. The relevance of each classifier to the current concept is evaluated by the generalization error when applying the classifier to the most recent data chunk. The relevance is employed as a weight applied to each classifier and the weighted classifiers are employed to make predictions for the current data chunk.

% \cite{Klinkenberg:2000} uses the $\xi \alpha$-estimators (based on leave-one-out estimation) to correct for concept drift while training an SVM. The authors use the maximum difference between any two elements of the Hessian (i.e. $R_\Delta^2 \ge \max_{x,x'} (\mathcal{K}(x,x)- \mathcal{K}(x,x'))$), $\xi$ the vector of training losses at the solution of the primal SVM training problem and $\alpha$ the solution of the dual to compute $d$.


% \begin{alignat}{1}
% \label{concept-drift}
% d = |\{i: (\alpha_i R_\Delta^2 + \xi_i) \ge 1 \}|
% \end{alignat}


% Since the document vectors are normalized to unit length, $R_\Delta^2 =1$ and it is proven in \cite{Joachims:2000} that $d$ is an approximate upper bound on the number of leave-one-out errors on the training set. The authors compute the $\xi \alpha$ estimate on the most recent $m$ examples of the streaming data for different window sizes and predict the window size with the lowest $\xi \alpha$ error. They show that this reduces concept drift.

% \cite{Liao:2009} uses Migratory Logistic Regression to learn concept drift between two data sets.  For a primary data point, $(x_i^p, y_i^p) \in \mathcal{D}^p$ they follow the  standard logistic regression to write, $P(y_i^p|\bold{x}_i^p; \bold{w}) = \sigma(y_i^p \bold{w}^T \bold{x}_i^p)$ where $\bold{w} \in \mathcal{R}^{d+1}$ is the column vector of weights and $\sigma$ is the sigmoid function. For an auxiliary data point $(x_i^a, y_i^a) \in \mathcal{D}^a$, they define

% \begin{alignat}{1}
% \label{migratory-lr}
% P(y_i^a|\bold{x}_i^a; \bold{w}, \mu_i) = \sigma(y_i^a \bold{w}^T \bold{x}_i^a + y_i^a \mu_i)
% \end{alignat}

% where $\bold{\mu}$ is a column vector of all auxiliary
% variables. The auxiliary variable $\mu_i$ is introduced to reflect the mismatch of $(x_i^a, y_i^a)$ with $\mathcal{D}^p$ and to control its participation in the learning of $\bold{w}$. A larger $y_i^a \mu_i$ makes $P(y_i^a|\bold{x}_i^a; \bold{w}, \mu_i)$ less sensitive to $\bold{w}$. To make the training more tractable the authors introduces constraints on $\mu_i$ and work out an analytical solution for $\bold{\mu}$ that allows them to alternatively train $\bold{w}$ and $\bold{\mu}$


\newpage

%Temporary working sheet
\subsection{Bug in the offline implementation (potentially online too)}
I think this is a bug that definitely impacts offline and likely online. Also, the paper formulation seem to be correct, i.e. paper and implementation are inconsistent.

This is our algorithm at step $t$ (as implemented in the offline code):
\begin{alignat}{1}
\min_{\beta} \delta F_{t-1}(\beta) + f_t(\beta) + \frac{\lambda}{2}||\beta||^2\\
F_{t-1}(\beta) = \frac{1}{2}\beta^T H_{t-1} \beta\\
H_{t-1} = X_{t-1}^T D_{t-1} X_{t-1} + Diag(\lambda) + \delta H_{t-2}
\end{alignat}
First part of the first equation $\delta F_{t-1}(\beta)$ is the discounted approximation of the objective function for the previous step $t-1$. In Bayesian view this is our prior based on the old data, it is simultaneously a posterior in the previous step, e.g. posterior in the step $t-1$ becomes prior in step $t$. This is not exact prior, we approximate it using the Laplace approximation (with Gaussian distribution). In the objective function it is simply expressed as a quadratic function (the second and third equations). The second part of the equation $f_t(\beta)$ is the objective based on the new data, the last part is the regularizer $\frac{\lambda}{2}||\beta||^2$ that corresponds to a Gaussian prior on all coefficients $Norm(0, Diag(1/\lambda))$.

I think equation (33) is where we have a bug - it should only have the first term (data component), not the regularization term (our global prior). Let's look at the first two steps of the algorithm:

{\bf STEP 0.}
\begin{alignat}{1}
\min_{\beta} f_0(\beta) + \frac{\lambda}{2}||\beta||^2
\end{alignat}
In Bayesian interpretation the posterior distribution of $\beta$ is used as a prior in the next iteration and is given by
\begin{alignat}{1}
P(\beta_0 | X_0) = Norm(\beta_0^*, H_0^{-1})\\
H_0 = X_0^T D_0(\beta_0^*) X_0 + Diag(\lambda)
\end{alignat}
Note: that it already includes $\lambda$ term. Then

{\bf STEP 1.}
\begin{alignat}{1}
\min_{\beta} f_1(\beta) + \frac{\delta}{2} \beta^T (X_0^T D_0(\beta_0^*) X_0 + Diag(\lambda))\beta   + \frac{\lambda}{2}||\beta||^2 = \\
\min_{\beta} f_1(\beta) + \frac{\delta}{2} \beta^T X_0^T D_0(\beta_0^*) X_0\beta + \frac{\lambda(1+\delta)}{2}||\beta||^2
\end{alignat}

The last term has $\lambda(1+\delta)$ which is effective increase of the regularization coefficient with every iteration of the algorithm. The series converge to $\lambda/(1-\delta)$, e.g. for our value of $\delta = 0.9$ it converges to $10\lambda$. We have two potential fixes that have slightly different interpretation:

{\bf Fix 1:} remove $\lambda$ from equation (31). This would result in $\lambda\delta$ regularizer. Effectively we keep forgetting not only the data, but our original prior as well.

{\bf Fix 2:} remove $\lambda$ from equation (33). This would result in a constant $\lambda$ regularizer. In this variant we are only forgetting the old data, but we never forget our original regularization prior.

{\bf Implementation aspect.}
This formulation problem caused a discrepancy in our offline and online algorithm. In offline we use static indexing of features (precomputed), in online we dynamically reindex features when a new previously unseen feature arrives. As a result in online implementation we start updating regularizaton coefficients for all features from start:
$$\lambda (1+ \delta (1 + \delta (1 +...))))$$
while for dynamic indexing we start this process after only after we observe the feature for the first time. This does not make sense, we will have different regularization values for different coefficients based on their first occurrence time. If we really wanted to use the current formulation, we would need to keep the effective value of $\lambda$ (that would depend on the iteration number) and apply it to all features, even newly observed. With {\bf Fix 2} we would not need to care about it.

\begin{alignat}{1}
\min_{\beta} f_t(\beta) + \delta F_{t-1}(\beta) + (1-\delta) \frac{\lambda}{2}||\beta||^2\\
F_{t-1}(\beta) = \frac{1}{2}\beta^t H_{t-1} \beta\\
H_{t-1} = X_{t-1}^T D_{t-1} X_{t-1} + \delta H_{t-2}\\
H_{t-1}^{full} = H_{t-1} + Diag(\lambda)
\end{alignat}


\newpage
